Deep 3D Capture: Geometry and Reflectance from Sparse Multi-View Images

We introduce a novel learning-based method to reconstruct the high-quality geometry and complex, spatially-varying BRDF of an arbitrary object from a sparse set of only six images captured by wide-baseline cameras under collocated point lighting. We first estimate per-view depth maps using a deep multi-view stereo network; these depth maps are used to coarsely align the different views. We propose a novel multi-view reflectance estimation network architecture that is trained to pool features from these coarsely aligned images and predict per-view spatially-varying diffuse albedo, surface normals, specular roughness and specular albedo. We do this by jointly optimizing the latent space of our multi-view reflectance network to minimize the photometric error between images rendered with our predictions and the input images. While previous state-of-the-art methods fail on such sparse acquisition setups, we demonstrate, via extensive experiments on synthetic and real data, that our method produces high-quality reconstructions that can be used to render photorealistic images.

==> Implementations.tex <==
%!TEX root = main.tex
\section{Implementation}\label{sec:implementaion}
\boldstart{Training data.}
% Similar to Xu et al~\cite{xu2019deep}, we first procedurally generate primitivie shapes such as cubes and cylinders, 
% and displace them with random height maps to increase the complexity. Afterwards we combine $  
We follow Xu et al.~\cite{xu2019deep} to procedurally generate complex scenes
by combining $1$ to $5$ primitive shapes such as cylinders and cubes displaced by random height maps.
We generate $20,000$ training scenes and $400$ testing scenes.
We divide the high-quality materials from the Adobe Stock dataset into a training and testing set,
and use them to texture the generated scenes separately. For each scene, 
following the proposed acquisition setup discussed in Sec.~\ref{sec:intro},
we render the images at 6 input views with a resolution of $512 \times 512$ using a physically based 
renderer with 1000 samples per pixel.  We also render the ground truth SVBRDF components and normal maps of each view. 
In total, we have $120000$ training images and $2400$ testing images. 

\boldstart{Network architecture.} For depth estimation, we use a 2D U-Net architecture 
for the feature extractor $\mc{F}$ and guidance map extractor $\mc{G}$. Each network comes 
with $2$ downsampling/upsampling blocks. The correspondence predictor $\mc{C}$ is a 3D U-Net 
with $4$ downsampling/upsampling blocks.  
In terms of SVBRDF estimation, both the encoder $\mc{E}$ and decoder $\mc{D}$ are 2D convolutional
neural networks, with $3$ downsampling layers in $\mc{E}$ and $3$ upsampling layers in $\mc{D}$.
We use group normalization~\cite{wu2018group} in all networks.
For more details on the network architecture, please refer to the supplementary materials.

\boldstart{Training details.}  All the networks are trained with 
Adam optimizer~\cite{kingma2014adam} for $50$ epochs with a learning rate of $0.0002$. 
The depth estimation networks are trained on cropped patches of $64 \times 64$ 
with a batch size of $12$, and the SVBRDF estimation networks are trained 
on cropped patches of $320 \times 320$ with a batch size of $8$. The networks are trained
on $4$ NVIDIA Titan 2080Ti GPUs.



